Image Matters: Visually modeling user behaviors using Advanced Model Server

In Taobao, the largest e-commerce platform in China, billions of items are provided and typically displayed with their images. For better user experience and business effectiveness, Click Through Rate (CTR) prediction in online advertising system exploits abundant user historical behaviors to identify whether a user is interested in a candidate ad. Enhancing behavior representations with user behavior images will help understand user's visual preference and improve the accuracy of CTR prediction greatly. So we propose to model user preference jointly with user behavior ID features and behavior images. However, training with user behavior images brings tens to hundreds of images in one sample, giving rise to a great challenge in both communication and computation. To handle these challenges, we propose a novel and efficient distributed machine learning paradigm called Advanced Model Server (AMS). With the well known Parameter Server (PS) framework, each server node handles a separate part of parameters and updates them independently. AMS goes beyond this and is designed to be capable of learning a unified image descriptor model shared by all server nodes which embeds large images into low dimensional high level features before transmitting images to worker nodes. AMS thus dramatically reduces the communication load and enables the arduous joint training process. Based on AMS, the methods of effectively combining the images and ID features are carefully studied, and then we propose a Deep Image CTR Model. Our approach is shown to achieve significant improvements in both online and offline evaluations, and has been deployed in Taobao display advertising system serving the main traffic.

==> body.tex <==
\section{Introduction}

%As the leading eCommercial Internet corporation, Alibaba also performs as large online advertiser. It is quite a challenging task to decide which advertise 
 
%Display advertising is an import revenue source of eCommercial Internet corporation like Alibaba. CTR prediction is the core task in advertising system\footnote{In this paper we focus on the CTR prediction, while the proposed methods can be easily generalized to other task such as CVR prediction}. 

%Deep learning based method is recently emerging. These systems largely rely on identifier(ID) based image. Content feature is referred less frequently, and usually treated as side information. 

%In this paper, we propose to 

Display advertising is a typical form of advertisement for Internet corporations such as Google, Alibaba and Tencent. Cost-per-click(CPC) is a widely adopted payment method for display advertising. In CPC mode, the ad publishers rank the candidate advertisements by eCPM(effective cost per mille)), which can be estimated by multiplying the bid price(a known value) by the (estimated) click through rate(CTR).  Such strategy makes CTR prediction the core task in the advertising system.

Traditional researches on CTR prediction largely focus on carefully designed feedback feature~\cite{yahoo1,yahoo2} and shallow models(\emph{e.g.}, Logistic Regression~\cite{richardson2007predicting}). In recent years, the deep learning based CTR prediction system emerged overwhelingly~\cite{zhang2017deep}. These methods mainly involve the sparse ID features(\emph{e.g.}, goods ID, user ID) of the described filed, while some literatures also explore the complementary effect of the content features(\emph{e.g.}, the user and item content representation)~\cite{lian2017cccfnet}. Among various content description features, images is intensively studied. For the images is the typical entry of website display advertising/recommender system(\emph{c.f.} Fig.~\ref{advertising_pipeline} for the scenario of our App) and images are direct depiction of the referred items.  

In fact, there are some pioneering works (\emph{cf.}~\cite{chen2016deep,mo2015image}) dedicating to explore the positive effects of image features in CTR prediction. They mainly focus on the image of ads. That is, to generate the visual description associate with the referred ad in the feedforward networks. As we know, joint modeling of the user and the advertisement is the core task in current CTR prediction system. It is natural to extend such visual auxiliary information to user modeling, since s user's interest is highly related to its behavior(\emph{c.f.} click) sequence, which is in itself an item and can be described by image information.  

%They mainly focus on the image of ads. However, as we know, joint modeling of the user and the advertisement is the core task in current CTR prediction system. What we concern most is whether a particular user will click on a particular ad. Therefore, it is nature extension 

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.95\linewidth]{fig/content_feat4.pdf}\\
  \caption{Joint training using both ID features and content features.}\label{key_contribution}
\end{figure}

To know is easy, but to do is difficult. There are two main problem in realizing this idea:

The first one (and the vital one) is how to build the system for industry application. Image is naturally heavy datasource, which makes our system quite sensitive to the quantity of images involved. Unfortunately, abundant user behavior inevitably bring huge number of related images. In our typical scenario, a single training sample involves one ad and one user, which associate to only one image for ad description while hundreds of images for user behavior description! That means, a trivial extension from user related image to user behavior images should tackle hundreds of times of storage and computing requirement. 

The second one is how to aggregate such user behavior images into an effective user description. User's behaviors may vary a lot, corresponding to various images, while should be encoded to a fix length representation vector. Furthermore, also the users have rich behavior according to its historical, only part of them are related to the current advertising display. In other word, different ad image would \emph{fire} different behavior images. Hence, to effectively modeling user behavior according to the given behavior image set remains challenging.

By addressing these two problems, here comes our contributions. In this paper, we propose a framework, named Deep Image CTR model(DICM), that jointly models the advertisement and the user with image content. To realize this framework:

\begin{enumerate}

\item We carefully design and build a highly efficient model training system and deploy a light weight online service, which manage to handle the newly involved user behavior images. In detail, we design a distributed GPU training system with multi(typically 20) workers, which utilizes the data parallelism and model parallelism. Ultimately, our training process with billions of sample is managed to complete within 24 hours, which means our online model can be daily updated. In this training system, a new distributed image processing architecture is highlighted. Specifically, we maintain a image pool, access the images by key-value manners and do in-place extracting of visual features. 

\item We systematically study the aggregation method for user behavior images. Several classical architecture is designed and empirically tested, and we find that simple sum pooling will lead to good tread-off considering online deployment and the double head attentive pooling with complementary query will lead to maximum performance in offline evaluation. 

\end{enumerate}

\section{Related work}

Our work is closely related to two kinds of techniques---CTR prediction in advertising/recommendation system and image representation in computer vision system, both of which have been developed independently for a long time.

The CTR prediction system actually evolves in two aspects. The first one is the progress on input features. Early research on CTR prediction lies on carefully designed low-dimensional statistic features, normally defined by votes of users' clicks, \emph{etc.}~\cite{yahoo1}, as well as their variant, \emph{e.g.}, the one with smoothing technique~\cite{yahoo2}. In recent years, large amounts of works try to build model based on high-dimensional sparse IDs feature(such as ad IDs or user IDs) to achieve more accurate description~\cite{zhou2017deep,WideandDeep}. The second one is the development of prediction model, from classical Logistical Regression~\cite{FTRL} and other shallow model such as decision trees~\cite{facebookCTR} to the well known multi-layer neural networks~\cite{zhou2017deep,WideandDeep}.

On the other hand, image representation, the core task of computer vision community, has attracted tremendous attention. Traditional work largely relies on handcraft feature extraction, among which GIST~\cite{oliva2001modeling}, HOG~\cite{dalal2005histograms}, \emph{etc.} give global description, while others such as Bag of Visual Word~\cite{sivic2003video}, VLAD~\cite{jegou2010aggregating}, Fisher vector~\cite{perronnin2010improving} choose the manners of local feature aggregation. However, recent progress on deep learning, especially CNN~\cite{alexnet,Simonyan2014Very,szegedy2015going,he2016deep}, motivates us to directly explore the raw pixels by multi layer non linear mapping. A common practice is to adopt well trained networks(without head part) as feature extractor and transfer to related task(\emph{e.g.}, ~\cite{ren2015faster,hariharan2015hypercolumns,wang2015action})

Our work lies in the intersection of CTR prediction and image description. In fact, there are some previous work trying to introduce image information in ad description. Cheng et al.~\cite{cheng2012multimedia} addresses the cold start problem by adding manually designed feature generated from images of ads. Mo et al.~\cite{mo2015image} extracts feature from ad images by CNN models pre-trained in classification task. Lynch et al. ~\cite{lynch2016images} introduce the visual information to overcome the misunderstanding of text-only representation in ranking system. Chen et al.~\cite{chen2016deep} proposes to involve images in an end-to-end network targeting on CTR prediction. These works only focus on the features generated from images of ads, but ignore that from images of goods appearing in the users' browsing history. 

\section{Background}

\subsection{Display advertising system}

For display advertising system, a basic unit, usually called \emph{impression}, is an incident that a specific ad is shown to a specific website user, in a specific scenario(viewing time, advertising position, \emph{etc.}). Its goal is to dig out appropriate ad that owns best predicted business index(\emph{cf.} eCPM) from the candidate group. 

Our display advertising platform serves tens of million of advertising, each representing an item on sale in our website. To handle such huge number of candidates for a given impression, the typical online system consists of three sequential modules, as shown in Fig.~\ref{advertising_pipeline} --- the \emph{matching} module which roughly selects around 4k candidates in an inverted file style, the successive \emph{preranking} module which shrinks the candidates to about 400 and at last the \emph{ranking} module give final selected advertising and feed them to the specified website position. All of these modules interact with the user description to give user-specified recommendation. The typical display advertising of our mobile app is as Fig.~\ref{advertising_pipeline}

%In this paper, we use the proposed DICM in both ranking and reranking phases, which share similar problem formulations. 
 
In this paper, we mainly focus on the \emph{ranking} module that most related to the quality of final result. In the next section, our system refers to the \emph{ranking} module unless specifically pointed. In the latter section, we show our DICM can extend to the \emph{preranking} phase with trivial change.

\begin{figure}

\centering

\begin{minipage}[c]{0.14\textwidth}
\includegraphics[width=1.0\linewidth]{fig/moble.pdf}
\caption{}\label{display_advertising}
\end{minipage}%
\begin{minipage}[c]{0.4\textwidth}
\includegraphics[width=1.0\linewidth]{fig/ali_advertising.pdf}
\caption{}\label{advertising_pipeline}
\end{minipage}

\end{figure}


\begin{comment}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.3\linewidth]{fig/moble.pdf}\\
  \caption{}\label{display_advertising}
\end{figure}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.8\linewidth]{fig/ali_advertising.pdf}\\
  \caption{}\label{advertising_pipeline}
\end{figure}

\end{comment}

%Holding hundreds of million website users as well as tens of million advertisers,  the display advertising system aims to assign given user 

%\section{Deep Image CTR Model for ranking}

%In this section, we focus on the \emph{ranking} module that most related to the quality of final result. 


\subsection{Problem Formulation}


In the \emph{ranking} module, our task is to predict precisely as possible the Click Through Rate(CTR) for the given impression. Following previous works~\cite{covington2016deep,chen2016deep,mo2015image,zhou2017deep}, we consider the CTR prediction as a two-class classification problem--- click as positive and non-click as negative. Feed gathered features, our networks model should infer a two dimensional vector (with one sum) to indicate the predicted CTR. In the training phase, the binary label whether an impression is clicked is provided, and the typical objective function is cross-entropy error~\cite{de2005tutorial}.

\subsection{Basic pipeline and architecture}

We set our baseline architecture as the popular Neural Collaborative Filtering~\cite{He2017neural} consisting of the ID feature embedding followed by the Multilayer Perceptron(MLP). Similar architectures are adopted by state-of-the-art CTR prediction systems such as $Wide\&Deep$~\cite{WideandDeep} and $DIN$~\cite{zhou2017deep}. Since our paper is exploring the effect of visual content information, we fix this part of structure and believe our method would benefit from any improvement of this backbone.

As illustrated in the left part of Fig.~\ref{Networks}, our baseline CTR prediction model is built on (sparse) ID features. These IDs belongs to various fields that describe different attributes of the ad, user, item and scenario context of the given sample impression. Depending on the its own property, the ID feature is either one-hot vector(\emph{e.g.}, ad id, user id, displaying position id) or with multiple none-zero entry(\emph{e.g}, user behavior id). The baseline model is divided to 2 parametric modules: the \emph{representer} which separately extracts each category of ID feature to one \emph{middle vector}, followed by the \emph{discriminator} which concatenates all \emph{middle vectors} to give final result. In our case, \emph{representer} is one layer linear transform, which is usually called \emph{embedding} and have efficient implementation due to the sparsity; while \emph{discriminator} is designed as 3 layer full connected networks.


\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.95\linewidth]{fig/architecture3.pdf}\\
  \caption{DICM network architecture for ranking}\label{Networks}
\end{figure}


\section{Joint modeling with images}

In this section, we introduce our methods -- the introduction of visual information on jointly description of ad and user. In the rest part of this paper, we simply use \emph{ad image} to denote the image representing the ad, and use \emph{user images} to denote a set of images representing one's historical behavior.

As illustrated in Fig.~\ref{Networks}, our system incorporate \emph{ad image} and \emph{user images} as two special feature field. They take image/images as input and process them by correspondent \emph{extractor} namely \emph{Adnet} and \emph{Usernet} respectively. 

The \emph{Adnet} can be viewed as an image feature \emph{extractor} which takes raw pixels of (resized) image as input and produces fixed length output vector with multi-layer net.  Similarly, the \emph{Usernet} is designed as  
    \emph{extractor} which process each of {user images} into vector,  followed by an \emph{aggregator} which pool all extracted vector of particular user into one fix-length vector. 
    
I the next subsection, we will first introduce the employed images, and then describe the \emph{extractor} and \emph{aggregator} detailedly. 

\subsection{Image as feature fields}

For ad, it is intuitive and has been successfully adopted~\cite{mo2015image,covington2016deep,cheng2012multimedia} that ad can be represented by the image viewed on the webpage as the entry of the ad. For user behavior, the representation image is not so straightforward, since there are various describable behaviors, such as  purchasing, favoring and clicking. In this paper we study the \emph{click} behavior, in the sense that \emph{click} is the most general user response that is able to bring rich descriptions. Another issue is  which image is related to \emph{click}. In this paper, we follow the natural sense to use the image one user was viewing when he/she did \emph{click} behavior. 
    
    
\subsection{Image feature extractor}

As illustrated in Fig.~\ref{Extractor}, the \emph{extractor} is designed to transfer the pixel-level visual information to middle-level description. In related works, the \emph{extractor} model is either pre-trained~\cite{mo2015image} or fully trained in end-to-end style~\cite{chen2016deep}. We consider it as an efficiency-effectiveness trade off, and propose a hybrid version: we split the whole net into \emph{fixed part} whose parameters is fixed and \emph{trainable part} that is involved in training.

The design of \emph{fixed part} is quite flexible and largely depends on the task. Here we select the first 14 layers of popular VGG16 net~\cite{Simonyan2014Very}, specifically, from Conv1 to FC6. This net will generate a 4096-D vector as input of \emph{trainable part}. For \emph{trainable part}, we simply use a 3-layer fully connected net, which is quite fast and can achieve enough fitting ability for industrial application. For simplicity of structure, we use symmetric design in which \emph{Adnet} and \emph{Usernet} share the same structure and leave the exploration of asymmetric structure as future work. 


\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.95\linewidth]{fig/extractor.pdf}\\
  \caption{Extractor architecture}\label{Extractor}
\end{figure}


\subsection{User behavior image feature aggregator}

The \emph{aggregator's} target is to model the user behavior by uncertain number of user vector, each representing one user behavior image, and finally give an fix dimensional description vector. In fact, there are many task on variable topic focusing on similar problem. For image retrieval/classification, one need to extract local feature(\emph{i.e.} SIFT~\cite{lowe1999object}) and use them to represent the whole image(\emph{c.f.} VLAD~\cite{jegou2010aggregating}, Fisher vector~\cite{perronnin2010improving} VLAD~\cite{jegou2010aggregating}). For sentence understanding, sentence can be modeled by aggregate the sequence of  words each of which is a vector by word embedding~\cite{bengio2003neural}. For Neural Machine Translation, the embedded word vector is aggregate by RNN~\cite{sutskever2014sequence}, CNN~\cite{Gehring2017conv} or Attentive method~\cite{Vaswani2017attention}. 

In this paper, we consider the following possible aggregation: 

\noindent\textbf{Flatten.} 

\noindent As illustrated in Fig.~\ref{Aggregator}(a), $N$ 12-Dim user image vectors are directly concatenated to $12 \times N$  middle vector. The capacity $N$ is fixed that user with more/less behaviors will be preprocessed by cutting off/padding.

\noindent\textbf{Sum/MaxPooling.} 

\noindent It is straightforward dimension-wise sum/max aggregating, with each entry of output middle vector is the summation/maximum of all corresponding entry of input vectors, as is shown in Fig.~\ref{Aggregator}(b). Sum/MaxPooling is widely adopted in image representation by local features~\cite{yang2009linear, wang2010locality}.

\noindent\textbf{AttenivePooling.} 

\noindent SumPooling can be viewed as equally weighed, corresponding to the assumption that each user behavior share equal importance in every impression scenario. However, it is not always the case. Many e-commercial site users have quantity of behaviors with large diversity. When equally weighted summed, \emph{user images} which are related to the ad would be inevitably interfered by the unrelated \emph{user images}. To alleviate this problem, the attentive weighted pooling, which has shown great success recently in Machine Translation~\cite{bahdanau2014neural, Vaswani2017attention}, is introduced.

As shown in Fig.~\ref{Aggregator}(c), the typical attentive mechanism consists three elements: the unique \emph{Query}, multiple vectors \emph{Key} each of which corresponds to a \emph{Value}. Query is designed as the context vector, which is spanned, concatenated with \emph{Key} one by one and feed into multi-layer fully connected networks to infer attentive weights. Finally, the \emph{Value} vector are sum-pooled according to the attentive weights.\footnote{There are different architectures for attentive weights generation and here we introduce the additive scheme.} In our case, we set context \emph{Query} as middle vectors from all involved feature fields but that of user behavior, including \emph{ad image middle vector} and middle vector of ID features. Both \emph{Key} and \emph{Value} are the \emph{user image middle vector} to be pooled.

\noindent\textbf{DoubleHead.}

\noindent As shown in Fig.~\ref{Aggregator}(d), we extend to multi-head(specifically double-head) structure which is introduced in ~\cite{Vaswani2017attention}. In detail, we jointly train 2 parametric attentive net with identical inputs, each of which generate an attentive weight vector. Then, the \emph{Value} is sum-pooled according to each of the attentive weights to two output vectors, which are concatenated to the double-width vector.  

\noindent\textbf{DoubleHead\_SplitQuery.}

\noindent As shown in Fig.~\ref{Aggregator}(e), it differs from \emph{DoubleHead} that \emph{Query} for each attentive module is a part of original. Its intuition is that different \emph{Query} would capture different context and derive different attention weight, thus generate pooled vectors with more complementarity. For example, the \emph{ad image} and the \emph{ad category id} will obviously motivate different attentions on the user behavior. 

\noindent\textbf{DoubleHead\_SplitQuery\_KeyAlign.}

\noindent As shown in Fig.~\ref{Aggregator}(f), compared with  \emph{DoubleHead\_SplitQuery}, it concatenate the corresponding \emph{user id vector}(before pooling) and \emph{user image vector} as \emph{Key}. We argue that the combined vector is more representative to the referred user behavior and generate more accurate attentive weights.   
\noindent

Besides the aforementioned architectures, \textbf{RNN} as an sequence encoder is also in the candidate list~\cite{sutskever2014sequence}. However, for RNN based method, the forward/backward time elapse will grow linearly with the behavior capacity, which is not affordable in our industry application. 


\begin{figure*}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.99\linewidth]{fig/aggregator.pdf}\\
  \caption{Aggregator architecture}\label{Aggregator}
\end{figure*}


\section{Hyper Parameter Server System}

As aforementioned, the main challenge of our proposed method is the huge quantity of images involved in user behavior. Image is not only big size datasource itself, but also relies on complex transformation in extracting semantic information for hight level understanding application such as CTR prediction. Therefore, our training system inevitably faces the heavy load of storage，computation and communication. To give concrete number,  a typical user would have over 200 behaviors during our statistic period，which means a single training sample will involve over 200 images, hundreds times more than that only involve ad by image. Let alone our training system should overtake billion scale training samples and finish model updating within one day, which is favorable for online advertising serving in our web.

Therefore, we carefully design a distributed GPU training system, which goes beyond the classical parameter server architecture~\cite{smola2010architecture, li2014scaling}, as well as its corresponding online serving pipeline. 

\subsection{Training system} 

Parameter Server(PS)~\cite{smola2010architecture, li2014scaling} is a widely adopted distributed architecture for large scale parametric machine learning problem. It consists of two node group: the \emph{worker group} contains a set of workers which do training on its assigned part of training samples(without mutually communication). Meanwhile, the server nodes in \emph{server group} jointly maintains a globally shared parameter pool which is usually with large size that can not repeatedly stored in worker node. During training, the worker node access/update the parameter pool though (key,value) data structure. 

Following previous work~\cite{zhou2017deep}, our baseline net(without image) is efficiently implemented as the PS-like architecture on GPU cluster. Such system randomly assign training data batch to worker nodes where network forward/backward are performed, while set the parameters of \emph{embedding} layer in \emph{server group} since its size far exceed the memory capacity of each worker. 

 However, when image features especially the tremendous user behavior related images are employed, the updating of training system is not trivial:
 
 The first issue is where to inject the image feature. Here instead of raw pixel, we focus on the image feature extracted by the \emph{fix part} of \emph{extractor}since its predecessor is not related to the model updating. A straightforward method is to add along with training batch the image feature which is involved. But such strategy is intractable since image feature will greatly expand the training batch (in our scenario, from 6M Bytes to 360M per batch, more than 50 times larger), which make it not affordable to IO and to store. Therefore, We turn to set the image feature as global common feature and store it into server node. Such strategy can greatly condense the total image feature storage, for some images frequently occur in different sample batches and only need to be saved as one copy in feature sharing style. 
 
 The second one is where to do the forward/backward operation. In typical PS architecture, all operations are performed separately in worker nodes, while server nodes simply response query in (key,value) manners and do not undertake any calculation task. However, this structure will obviously bring heavy load of communication between worker and server, since the image feature is high dimensional. A solution is move some operation to server node and so as to communicate the processed vector in the "bottleneck" point of the whole network. Hence, we propose to update the \emph{server group} to the \emph{advanced feature service} by equipping the server node with the (parametric) operator. Specifically, we assign the \emph{trainable part} of \emph{extractor} for both \emph{Adnet} and \emph{Usernet} to the server node. This part of network is only related to the input image feature separately and does not interact with other ID feature, thus can be conveniently calculated in on-site manner. 
 
 Fig.~\ref{system} illustrate our designed distributed GPU training system which highlights the \emph{advanced feature service}. The input training data does not contain the referred image features, but only record their IDs. Instead, the image feature(preprocessed by \emph{fix part} of \emph{extractor}) for both \emph{ad image} and \emph{user images} are partition-wise stored in \emph{advanced feature service} node group with id ad key. Similar to worker node, the \emph{advanced feature service} node keeps the parametric operation --- the \emph{image extractor}. In forward phrase of training, when receiving query image id, the \emph{advanced feature service} fetches corresponding image feature from database and directly performs the \emph{extractor} processing, and then sent the processed vector to \emph{discrimination service} module. In backward, the \emph{advanced feature service} receives the gradient from \emph{model service} and update the parameter of \emph{extractor} with back propagation. 
 
 Besides reducing the communication load by shrinking image feature vector(typically from 4096-D to 12-D, over 300 times compression ratio), we further claim another benefit of such design is that queries from different worker node within one training iteration can be naturally merged and share the \emph{extractor} process, which greatly reduces the computation load.
 

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.99\linewidth]{fig/system3.pdf}\\
  \caption{System overview}\label{system}
\end{figure}



\begin{comment}
\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.99\linewidth]{fig/system2.pdf}\\
  \caption{System overview}\label{system}
\end{figure}

\end{comment}


\subsection{Inference and online deployment}

As we know, a complete framework for real word advertising includes both training phase that generate models and the online deployment that use model  to give CTR prediction for advertise engine. In this subsection, we briefly introduce our online deployment. 

For our baseline model(without image), the deployment is trivial. We gather all learnt parameters, including the parametric embedding vector for each ID and the parameters of full connected layers, and use them to build a PS-like predictor that access the embed parameter vector in key-value matter from shared storage. 

As it to the deployment of image involving model, our design strategy is to "hide" the image extractor and reuse the ID based predictor. To this end, we first process all involved \emph{ad image} and \emph{user images} by the trained \emph{extractor}(including \emph{trainable part}), and then append the processed image middle vector(12-D in our system) to the ID embedding vector set. Since the input sample only provide image IDs, then the extracted image vector can also be fetched by K-V manner. In other word, the image vector is totally equally treated as ID feature by using processed image vector to replace the learned ID embedding parameter vector.

Such design guarantee the image based model share similar online serving elapse, which is also verified by our online experiment. 

\section{Training details}

For baseline model, we follow the online platform configuration and use 27 categories of ID features including user profiles, user behavior, ad description and scenario description. Since we focus on the
comparison of image content feature and the corresponding ID feature, we do not utilize extra tricks such as cross-product feature.  To speed up training and reduce storage cost, we follow the common-feature technique~\cite{zhou2017deep,chen2016deep}. In detail, we gather samples corresponding to identical user to form sample groups which share user relevant feature as common-feature.
%since user relevant feature costs much higher than others.

For training, we employ a 20-GPU cluster, on which the \emph{advanced feature service} and \emph{discrimination service} runs in a time-sharing way. To further speed up the time-consuming image fetching, we cache images with high frequency in memory, and design the asynchronous pre-fetch process. We set the batch size to 3,000 per parallel node, thus the overall batch size is 60,000. To describe user behavior, we select the \emph{click} behavior of one specific user in the past 14 days. Since raw data from real system is noisy, we pick \emph{typical click behavior} according to the visiting elapsed time, visiting frequency, etc. On average, each user have 32.6 behaviors according to statistics, and there are altogether 200 million unique images involved in training task.

We use PReLU~\cite{he2015delving} as the activation for each layer since we empirically find its superiority. We use Adam~\cite{kingma2014adam} as parameter optimizer, with the learning rate initialized to 0.001 and decayed by 0.9 after each 24,000 sample batches.


\subsection{Partial warm-up}

Due to the different data representation, the difficulties of training baseline net, \emph{Adnet} and \emph{Usernet} are totally different, thus make them hard to converge at the same speed. The \emph{Adnet} and \emph{Usernet} are relatively deep to extract highly non-linear image feature, which need intense training. Meanwhile, the embedding net of baseline net is quite shallow but with large quantity of parameters, thus is prone to get overfitting. Therefore, it is wise to design the learning scheme that update \emph{Adnet} and \emph{Usernet} more frequently than baseline net. Here we propose the \emph{partial warm-up}. In detail, we use pre-trained (but with training data of different date) model as initialization of \emph{Adnet} and \emph{Usernet} and randomly initialize the rest part of model. Benefit from the daily update scheme of our system, we can use the trained model of last day as initialization without any extra cost. We find it works well and does not need require any change in the training phase.


\section{Deep Image CTR Model for preranking}

\section{Experiments}




\subsection{}

\subsection{}

\subsection{}

\subsection{}


\section{Conclusion}



==> ch_back.tex <==
\section{Background}



\subsection{Display advertising system} \label{ch_display_adv_sys}

\begin{figure}

\centering

\begin{minipage}[c]{0.14\textwidth}
\includegraphics[width=1.0\linewidth]{fig/moble.pdf}
\caption{Typical display ad on App of Taobao}\label{display_advertising}
\end{minipage}%
\begin{minipage}[c]{0.4\textwidth}
\includegraphics[width=1.0\linewidth]{fig/ali_advertising.pdf}
\caption{Display advertising pipeline}\label{advertising_pipeline}
\end{minipage}

\end{figure}

For display advertising system, a basic unit, usually called and \emph{impression}, is an incident that a specific ad is shown to a specific website user, in a specific scenario(viewing time, advertising position, \emph{etc.}). Its goal is to dig out appropriate ad that owns best predicted business index(\emph{cf.} eCPM) from the candidate group. 

Our display advertising platform serves tens of millions of advertising, each representing an item on sale in our website. To handle such huge number of candidates for a given impression, the typical online system consists of three sequential modules, as shown in Fig.~\ref{advertising_pipeline} --- the \emph{matching} module which roughly selects around 4k candidates in an inverted file style, the successive \emph{Pre-rank} module which shrinks the candidates to about 400 and at last the \emph{Rank} module give final selected advertising and feed them to the specified website position. All of these modules interact with the user description to give user-specified recommendation. The typical display advertising of our mobile app is as Fig.~\ref{display_advertising}

%In this paper, we use the proposed DICM in both ranking and reranking phases, which share similar problem formulations. 
 
In this paper, we mainly focus on the \emph{Rank} module that most related to the quality of final result. In the next section, our system refers to the \emph{Rank} module unless specifically pointed. In the latter section, we show our DICM can extend to the \emph{Pre-rank} phase with trivial change.


\begin{comment}
\begin{figure}
\subfigure[]{
\label{ad_gauc} %% label for first subfigure
\includegraphics[width=0.25\linewidth]{fig/moble.pdf}}
\subfigure[]{
\label{ad_user_gauc} %% label for first subfigure
\includegraphics[width=0.72\linewidth]{fig/ali_advertising.pdf}}
\caption{Comparison on ad/user ID(s) and ad/user image(s) (\emph{prefix} denotes basic ID+ad ID+ad image)}
\label{fig:gauc} %% label for entire figure
\end{figure}

\end{comment}






\begin{comment}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.3\linewidth]{fig/moble.pdf}\\
  \caption{}\label{display_advertising}
\end{figure}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.8\linewidth]{fig/ali_advertising.pdf}\\
  \caption{}\label{advertising_pipeline}
\end{figure}

\end{comment}

%Holding hundreds of million website users as well as tens of million advertisers,  the display advertising system aims to assign given user 

%\section{Deep Image CTR Model for ranking}

%In this section, we focus on the \emph{ranking} module that most related to the quality of final result. 


\subsection{Problem Formulation}\label{ch_problem}


In the \emph{Rank} module, our task is to predict precisely as possible the Click Through Rate(CTR) for the given impression. Following previous works~\cite{covington2016deep,chen2016deep,mo2015image,zhou2017deep}, we consider the CTR prediction as a two-class classification problem--- click as positive and non-click as negative. Feed gathered features, our networks model should infer a two dimensional vector (with one sum) to indicate the predicted CTR. In the training phase, the binary label whether an impression is clicked is provided, and the typical objective function is cross-entropy error~\cite{de2005tutorial}.

\subsection{Basic pipeline and architecture}

We set our baseline architecture(called \emph{BasicNet}) as the popular Neural Collaborative Filtering~\cite{He2017neural} consisting of the ID feature embedding followed by the Multilayer Perceptron(MLP). Similar architectures are adopted by state-of-the-art CTR prediction systems such as $Wide\&Deep$~\cite{WideandDeep} and $DIN$~\cite{zhou2017deep}. Since our paper is exploring the effect of visual content information, we fix this part of structure and believe our method would benefit from any improvement of this backbone.

As illustrated in the left part of Fig.~\ref{Networks}, our baseline CTR prediction model is built on (sparse) ID features. These IDs belongs to various fields that describe different attributes of the ad, user, item and scenario context of the given sample impression. Depending on the its own property, the ID feature is either one-hot vector(\emph{e.g.}, ad id, user id, displaying position id) or with multiple none-zero entry(\emph{e.g}, user behavior id). The baseline model is divided to 2 parametric modules: the \emph{representer} which separately extracts each category of ID feature to one \emph{middle vector}, followed by the \emph{discriminator} which concatenates all \emph{middle vectors} to give final result. In our case, \emph{representer} is one layer linear transform, which is usually called \emph{embedding} and have efficient implementation due to the sparsity; while \emph{discriminator} is designed as 3 layer fully connected networks.


\begin{figure*}
  \centering
  % Requires \usepackage{graphicx}
  %\includegraphics[width=0.95\linewidth]{fig/architecture4.pdf}\\
  \includegraphics[width=0.95\linewidth]{fig/graf_fig2.pdf}\\
  \caption{DICM network architecture for \emph{Rank}}\label{Networks}
\end{figure*}







==> ch_detail.tex <==
\section{Implementation Details}

%We discuss several important items for system implementation. 


%\subsection{Image feature \emph{extractor}}

%The \emph{extractor} is designed to transfer the pixel-level visual information to middle-level description. In related works, the \emph{extractor} model is either pre-trained~\cite{mo2015image} or fully trained in end-to-end style~\cite{chen2016deep}. We consider it as an efficiency-effectiveness trade off, and propose a hybrid version: we split the whole net into \emph{fixed part} whose parameters are fixed and \emph{trainable part} that is involved in training.


\subsection{Inference and online deployment}

Our DICM is deployed in Taobao's display advertising engine. For Embedding\&MLP model (without images), 
the online server runs like the forward process of training system by query embedding parameters in global pool. 

As to the deployment of image involving model, our design the online strategy is to hide the image embedding model and change it to ID embedding mechanism. To this end, we preprocess all images by learned embedding model in offline style when training ends, and treat the embedded image vector as ID embedding parameter in the online process.
Note that the newly involved images can be embedded and added directly, which alleviates the cold start problem of ID features.
Benefitting from this trick, our DICM increases the response time over the baseline in a tolerable degree, from 21 millisecond to 24 millisecond for each advertising PV request.


%Such design guarantees the image based model share similar online serving elapse, which is also verified by our online experiment. 


%the deployment is 



%For Embedding\&MLP model(without images), the deployment is trivial. We gather all learnt parameters, including the parametric embedding vector for each ID and the parameters of full connected layers, and use them to build a PS-like predictor that access the embed parameter vector in key-value matter from shared storage. 


%As we know, a complete framework for real word advertising includes both training phase that generate models and the online deployment that use model  to give CTR prediction for advertise engine. In this subsection, we briefly introduce our online deployment. 



%As to the deployment of image involving model, our design strategy is to "hide" the image extractor and reuse the ID based predictor. To this end, we first process all involved \emph{ad image} and \emph{user images} by the trained \emph{extractor}(including \emph{trainable part}), and then append the processed image middle vector(12-D in our system) to the ID embedding vector set. Since the input sample only provide image IDs, then the extracted image vector can also be fetched by K-V manner. In other word, the image vector is totally equally treated as ID feature by using processed image vector to replace the learned ID embedding parameter vector.

%Such design guarantees the image based model share similar online serving elapse, which is also verified by our online experiment. 



\subsection{Partial warm-up}\label{warm-up}

%Due to the different data representation, the difficulties of training \emph{BasicNet}, \emph{AdNet} and \emph{UserNet} are totally different, thus make them hard to converge at the same speed. The \emph{AdNet} and \emph{UserNet} are relatively deep to extract highly non-linear image feature, which need intense training. Meanwhile, the embedding part of \emph{BasicNet} is quite shallow but with large quantity of parameters, thus is prone to get overfitting. Therefore, it is wise to design the learning scheme that update \emph{AdNet}, \emph{UserNet} and the MLP part of \emph{BasicNet} more frequently than the Embedding part of \emph{BasicNet}. Here we propose the \emph{partial warm-up}. In detail, we use pre-trained (but with training data of different date) model as initialization of \emph{AdNet} and \emph{UserNet} and the MLP part of \emph{BasicNet}, while randomly initialize the rest embedding part. Benefit from the daily update scheme of our system, we can use the trained model of last day as initialization without any extra cost. We find it works well and does not need require any change in the training phase.


Parameter initialization is widely used in parametric learning task. Benefitting from the daily update scheme of our system, we can use the trained model of last day as initialization without any extra cost. It is observed that the ID embedding part is quite shallow but with large large size of parameters, thus is prone to get overfitting. So we propose the \emph{partial warm-up} technique. In detail, we use pre-trained (but with training data of different date) model as initialization of all parts except ID embedding (\emph{i.e.} image embedding model, extractor and MLP part), while randomly initialize the ID embedding part. 
 
%We empirically study the partial warm-up stragtegy with setting introduced in Sec.~\ref{experiment_setting}. 

We empirically study the partial warm-up by comparing the strategy of non warm-up, partial warm-up (except embedding part) and full warm-up. As shown in Table~\ref{tab:warm-up}, partial warm-up performs best, whereas that with all model initialized get collapsed. It serves our proposal that the embedding part should not be initialized to avoid overfitting.

%We study(with setting introduced in Sec.~\ref{experiment_setting}) the partial warm-up by successively adding

%the following modules of our model in the initialization set: 

%the \emph{Adnet} and \emph{Usernet}, the \emph{Basenet}. As shown in Table~\ref{tab:warm-up}, initializing $Adnet + Usernet$ performs best, while that with all models initialized get collapsed. It serves our proposal that embedding part should not be initialized to avoid overfitting. 

\begin{comment}
Since we are using the model of last day to initialize, it is essential to check the long-term effect of such periodical strategy. We report the successive 7 days' comparison of offline training in our real system, depicted at Table~\ref{tab:structure}. We see the consistent gap of the GAUC between the strategies of with and without partial warm-up. 
\end{comment}


\begin{table}[htbp]
\centering
\begin{tabular}{|c||c|c|c|}
  \hline
  warm-up strategy &    Non    &  \textbf{Partial} & Full\\ \hline
  GAUC     &  0.6260  & \textbf{0.6283}   & 0.6230  \\ 
  \hline
\end{tabular}
\caption{Comparison of warm-up strategy}
\label{tab:warm-up}
\end{table}


\begin{comment}

\begin{table}[htbp]
\centering
\begin{tabular}{l c}
  \toprule
   warm-up module              & GAUC \\  \midrule
   Non                         & 0.6260  \\ 
   \textbf{Adnet+Usernet}      & \textbf{0.6272}  \\
   \textbfAll  & 0.6230  \\
 \bottomrule
   
\end{tabular}
\caption{result of partial warm-up}
\label{tab:warm-up}
\end{table}

\end{comment}

\begin{comment}


\begin{table}[htbp]
\centering
\begin{tabular}{l c}
  \toprule
   warm-up module              & GAUC \\  \midrule
   Non                         & 0.6260  \\ 
   Adnet+Usernet                    & 0.6272  \\
   \textbf{Adnet+Usernet + MLP}              & \textbf{0.6283}  \\
   Adnet+Usernet + MLP + Embednet.  & 0.6230  \\
 \bottomrule
   
\end{tabular}
\caption{result of partial warm-up}
\label{tab:warm-up}
\end{table}

\end{}

\begin{comment}
\begin{table*}[!h]
\centering
\begin{tabular}{|c||c|c|c|c|c|c|c|}
  \hline
  Day      &  1 &  2 & 3  & 4 & 5 & 6 & 7\\ \hline
  Without warm-up    &   0.xxxx  & 0.xxxx   & 0.xxxx  & 0.xxxx  & 0.xxxx & 0.xxxx & 0.xxxx   \\ 
  With warm-up       &   0.xxxx  & 0.xxxx   & 0.xxxx. & 0.xxxx  & 0.xxxx & 0.xxxx & 0.xxxx  \\ 
  \hline
  
\end{tabular}
\caption{Long-term evaluation of partial warm-up}
\label{tab:structure}
\end{table*}
\end{comment}




